Good Subnetworks Provably Exist: Pruning via Greedy Forward Selection

Recent empirical works show that large deep neural networks are often highly redundant and one can find much smaller subnetworks without a significant drop of accuracy. However, most existing methods of network pruning are empirical and heuristic, leaving it open whether good subnetworks provably exist, how to find them efficiently, and if network pruning can be provably better than direct training using gradient descent. We answer these problems positively by proposing a simple greedy selection approach for finding good subnetworks, which starts from an empty network and greedily adds important neurons from the large network. This differs from the existing methods based on backward elimination, which remove redundant neurons from the large network. Theoretically, applying the greedy selection strategy on sufficiently large {pre-trained} networks guarantees to find small subnetworks with lower loss than networks directly trained with gradient descent. Our results also apply to pruning randomly weighted networks. Practically, we improve prior arts of network pruning on learning compact neural architectures on ImageNet, including ResNet, MobilenetV2/V3, and ProxylessNet. Our theory and empirical results on MobileNet suggest that we should fine-tune the pruned subnetworks to leverage the information from the large model, instead of re-training from new random initialization as suggested in \citet{liu2018rethinking}.

==> experiment.tex <==
\section{Experiments}

In this section, 
we first apply our proposed algorithm on ImageNet~\citep{deng2009imagenet} on various models, e.g. ResNet~\citep{he2016resnet}, MobileNetV2~\citep{sandler2018mobilenetv2} and ProxylessNet~\citep{cai2018proxylessnas}.
We then demonstrate finetuning is better than training from scratch for small models, e.g. MobileNetV2.
It suggests that it is important to finding important weights from a large network when we aim to obtain an extreme small network.
Finally, 
we display experimental results on CIFAR10.

\begin{table*}[htbp!]
    \centering
    \begin{tabular}{l|l|c|c|c}
        \hline
        Model & Method & top-1 acc & Size (M) & FLOPS \\
        \hline
        \multirow{8}{*}{ResNet34} & \citet{he2016resnet} & 73.4 & - & 3.67G \\
        \cline{2-5}
        & \citet{li2016pruning} & 72.1 & - & 2.79G \\
        & \citet{liu2018rethinking} & 72.9 & - & 2.79G \\
        % \cline{2-5}
        & \citet{dong2017more} & 73.0 & - & 2.75G \\
        & FW-A & \bf{73.5} & - & \bf{2.64G} \\
        \cline{2-5}
        & SFP~\citep{he2018soft} & 71.8 & - & 2.17G \\
        & FPGM~\citep{he2019filter} & 72.5 & - & 2.16G \\
        % \cline{2-5}
        & FW-B & \bf{72.9} & - & \bf{2.07G} \\
        \hline
        \multirow{9}{*}{MobileNetV2} & \citet{sandler2018mobilenetv2} & 72.0 & 3.5 & 300M \\
        & FW-A & \bf{71.7} & 2.9 & 217M \\
        \cline{2-5}
        & \citet{sandler2018mobilenetv2} (Unif) & 70.4 & 2.6 & 210M \\
        & AMC~\citep{he2018amc} & 70.8 & 2.6 & 210M \\
        % & LeGR~\citep{chin2019legr} & 71.4 & - & 210M \\
        & FW-B & \bf{71.1} & 2.6 & \bf{200M} \\
        \cline{2-5}
        & \citet{sandler2018mobilenetv2} (Unif) & 66.7 & 2.3 & 165M \\
        & ThiNet~\citep{luo2017thinet} & 63.4 & - & 165M \\
        & DPL~\citep{zhuang2018dpl} & 64.2 & - & 165M \\
        & LeGR~\citep{chin2019legr} & 69.4 & - & 150M \\
        & FW-C & \bf{70.2} & 2.3 & 169M \\
        \hline
        \multirow{1}{*}{ProxylessNet-Mobile} & \citet{cai2018proxylessnas} & 74.6 & 4.1 & 324M \\
        \hline
    \end{tabular}
    
    \caption{Top-1 and Top-5 errors for different benchmark models, e.g.  ResNets~\citep{he2016resnet}, MobileNetV2~\citep{sandler2018mobilenetv2} on ImageNet2012~\citep{deng2009imagenet}. We apply different pruning methods and show their final performance.}
    \label{tab:imagenet}
\end{table*}

\subsection{Finding Sub-Networks on ImageNet}

\paragraph{Training Details}
During finetuning, 
we use the standard SGD optimizer with Nesterov momentum 0.9 and
weight decay $5 \times 10^{-5}$. 
We initialize the learning rate from $0.01$ and decay the learning rate with the cosine schedule~\citep{loshchilov2016cosine}.
The sub network is finetuned for 150 epochs with batch size 512 on 4 GPUs.

\paragraph{Results}
Table ~\ref{tab:imagenet} reports the top1 accuracy, FLOPs and model size of sub-networks derived from the full networks.
We test our algorithm on two standard benchmarks, 
ResNet-34 and MobileNetV2.
We further apply our algorithm to some recent proposed models, e.g ProxylessNet.
We demonstrate that our algorithm can outperform all the other pruning methods, and can be applied to mobile models.

Table ~\ref{tab:imagenet} demonstrate the results on ResNet-34 and MobileNetV2.
Comparing with prior art, 
our algorithm is superior to all the prior art that reports on ResNet-34 and MobileNetV2.
On ResNet-34, 
we obtain even better top1 accuracy ($73.4\% \longrightarrow 73.5\%$ ) than the full size network
while reduce the FLOPs from 3.67G to 2.64G.

Different from ResNet or other standard structures, 
it is hard to pruning MobileNetV2 on ImageNet for most of the traditional pruning algorithms~\citep{chin2019legr}.
As shown in Table~\ref{tab:imagenet}, 
most of the popular algorithms fails to outperform a naive baseline, 
uniformly reducing the number of channels for each layer.
Our proposed algorithm, however, improve the performance of extreme small network by a significant margin.
The subnetwork with 217M FLOPs obtains $71.7\%$ top1 accuracy, which only drops the accuracy of the full size network a little bit ($72.0\% \longrightarrow 71.7\%$).
Our subnetwork with 169M FLOPs can achieve $70.2\%$ top1 accuracy, 
which improve the $66.7\%$ top1 accuracy of uniform baselines, 
and also improve the previous state-of-the-art result, $69.4\%$ top1 accuracy with 150M FLOPs.

{\color{red}{to do: More results on other structures, draw a figure to show the trade-off between flops and acc}}

\subsection{Rethinking the Value of Finetuning}
Recently, ~\citet{liu2018rethinking} finds out that 
for ResNet, VGG~\citep{simonyan2014vgg} and other structures, 
training the pruned structure from scratch can achieve better performance than finetuning.
However, 
in this work, 
we empirically find that this claim is not true for mobile models, 
e.g. MobileNetV2.

As shown in Table~\ref{tab:rethink}, 
for these mobile models, 
finetuning can outperform training from scratch by a large margin.
For the FW-C structure, 
training from scratch will break $70.2\%$ top1 accuracy to $67.3\%$ top1 accuracy.
This fact suggests that finding a good initialization for the mobile models is significantly important.

\subsection{Rethinking the Value of Training Large Networks}
Most of the existing pruning algorithms apply the $L_p$ regularization on the large network during training ~\citep{li2016pruning, he2019filter}.
On large enough models or small datasets, 
these algorithms will not break the performance of the large networks and can find important channels.

However, for mobile models, researchers have found that
few of the channels can be pushed to have small norms, 
and stronger regularization can drop the performance a lot~\citep{chin2019legr}.

Unlike these approaches, 
~\citet{frankle2018lottery} tries to find a good initialization of a small network from the large network.
However, the empirical results of ~\citep{frankle2018lottery} and its variants are not as strong as standard pruning algorithms 
and do not use the weight of the pre-trained large networks.

To some extent,
our algorithm extends the idea of ~\citet{frankle2018lottery}.
We try to find a good initialization of the small network 
from the weights of a pre-trained large network.
We use the pre-trained large networks, 
as it has already memorized the training data~\citep{zhang2016understanding} and had good generalization~\citep{du2018gradient}.
Our algorithm has strong empirical results
and also have theoretical guarantees that
we can approximate the output of the large network with a subset of the neurons with $\epsilon$-bounded error.


\begin{table}[htbp!]
    \centering
    \begin{tabular}{l|l|c|c}
        \hline
        Model & FLOPs & Train From Scratch & Finetune \\
        \hline
        FW-A & 217M & 69.8 & 71.7 \\
        \hline
        FW-C & 169M & 67.3 & 70.2 \\
        \hline
    \end{tabular}
    
    \caption{Top1 accuracy on MobileNetV2 on ImageNet.}
    \label{tab:rethink}
\end{table}


\subsection{Finding Sub-Networks on CIFAR10}

In this subsection, 
we display the results of applying our proposed algorithm to various model structures on CIFAR10.

{\color{red}{to do: some results on cifar}}

